Quantum commitments and signatures without one-way functions

In the classical world, the existence of commitments is equivalent to the existence of one-way functions. In the quantum setting, on the other hand, commitments are not known to imply one-way functions, but all known constructions of quantum commitments use at least one-way functions. Are one-way functions really necessary for commitments in the quantum world? In this work, we show that non-interactive quantum commitments (for classical messages) with computational hiding and statistical binding exist if pseudorandom quantum states exist. Pseudorandom quantum states are sets of quantum states that are efficiently generated but their polynomially many copies are computationally indistinguishable from the same number of copies of Haar random states [Ji, Liu, and Song, CRYPTO 2018]. It is known that pseudorandom quantum states exist even if $\BQP=\QMA$ (relative to a quantum oracle) [Kretschmer, TQC 2021], which means that pseudorandom quantum states can exist even if no quantum-secure classical cryptographic primitive exists. Our result therefore shows that quantum commitments can exist even if no quantum-secure classical cryptographic primitive exists. In particular, quantum commitments can exist even if no quantum-secure one-way function exists. In this work, we also consider digital signatures, which are other fundamental primitives in cryptography. We show that one-time secure digital signatures with quantum public keys exist if pseudorandom quantum states exist. In the classical setting, the existence of digital signatures is equivalent to the existence of one-way functions. Our result, on the other hand, shows that quantum signatures can exist even if no quantum-secure classical cryptographic primitive (including quantum-secure one-way functions) exists.

==> crypt_Preliminaries.tex <==
\section{Preliminaries}
\subsection{Quantum information}
The fidelity $F(\rho,\sigma)$ between two states $\rho,\sigma$ is
defined by 
\begin{eqnarray*}
F(\rho,\sigma):=\Big(\mbox{Tr}\sqrt{\sqrt{\sigma}\rho\sqrt{\sigma}}\Big)^2.
\end{eqnarray*}
If $\sigma=|\sigma\rangle\langle\sigma|$,
$F(\rho,\sigma)=\langle\sigma|\rho|\sigma\rangle$.
For any bipartite states $\rho_{AB},\sigma_{AB}$,
$F(\rho_{AB},\sigma_{AB})\le F(\rho_A,\sigma_A)$,
where $\rho_A=\mbox{Tr}_B(\rho_{AB})$
and $\sigma_A=\mbox{Tr}_B(\sigma_{AB})$.
For any states $\rho,\sigma,\xi$,
\begin{eqnarray*}
F(\rho,\xi)+F(\sigma,\xi)\le 1+\sqrt{F(\rho,\sigma)}.
\end{eqnarray*}

\if0
For any states $\{\rho_x\}_x,\{\sigma_x\}_x$ and any probability distribution $\{p_x\}_x$,
\begin{eqnarray*}
\sqrt{F\left(\sum_xp_x\rho_x,\sum_xp_x\sigma_x\right)}
\ge \sum_xp_x\sqrt{F(\rho_x,\sigma_x)}.
\end{eqnarray*}
\fi



\subsection{Cryptography}
\begin{definition}[PRS generator]
A pseudorandom state generator is a pair of algorithms $(\KeyGen,\StateGen)$ as follows:
\begin{description}
\item[$\KeyGen(1^n)\to k$:]$ $
It is a PPT algorithm that, on input $1^n$, outputs a key $k\in\{0,1\}^n$.
\item[$\StateGen(1^n,k)\to |\phi_k\rangle$:]$ $
It is a QPT algorithm that, on input $1^n$ and $k$, outputs an $m$-qubit quantum state $|\phi_k\rangle$ 
with $m=\poly(n)$.
\end{description}

We require the following security: 
for any polynomial $t$ and any non-uniform QPT adversary $\cA$ there exists a negligible function $\negl$
such that for all $n$
\begin{eqnarray*}
\left|\Pr_{k\leftarrow \KeyGen(1^n)}\left[\cA(|\phi_k\rangle^{\otimes t(n)})=1\right]
-\Pr_{|\psi\rangle\leftarrow \mu}\left[\cA(|\psi\rangle^{\otimes t(n)})=1\right]\right|\le \negl(n),
\end{eqnarray*}
where $\mu$ is the Haar measure on $S(2^m)$.
\end{definition}

\begin{remark}
In this paper, we assume $m\ge 3n$.
\end{remark}

\begin{definition}[Non-interactive commitment]
A non-interactive commitment is the following protocol.
\begin{description}
\item[Commit phase:]$ $
Let $b\in\{0,1\}$ be the bit committed. 
The sender generates a quantum state $|\psi_b\rangle_{RC}$, and 
sends the register $C$ to the receiver.
\item[Reveal phase:]$ $
The sender sends $b$ and the register $R$ to the receiver.
The receiver checks whether the state of the registers $R$ and $C$ is
$|\psi_b\rangle$ or not.
If so, the receiver outputs $b$. If not, the receiver outputs $\bot$.
\end{description}
As the security, we require the following:
\end{definition}

\begin{definition}[Computational hiding]
Let us consider the following security game, $\mathsf{Exp}(b)$, with the parameter $b\in\{0,1\}$
between a QPT challenger $\cC$ and a QPT adversary $\cA$.
\begin{enumerate}
\item
$\cC$ generates 
$|\psi_b\rangle_{RC}$ 
and sends the register $C$ to $\cA$.
\item
$\cA$ outputs $b'\in\{0,1\}$,
which is the output of the experiment.
\end{enumerate}
We say that the commitment scheme is computationally hiding if
\begin{eqnarray*}
\left|\Pr[\mathsf{Exp}(0)=1]-\Pr[\mathsf{Exp}(1)=1]\right|\le \negl(\lambda).
\end{eqnarray*}
\end{definition}

\begin{definition}[Statistical sum-binding]
Let us consider the following security game between a QPT challenger $\cC$ and an unbounded adversary
$\cA$ with the parameter $b\in\{0,1\}$.
\begin{enumerate}
\item
$\cA$ generates a state $|\Psi\rangle_{ERC}$, and sends the register $C$ to $\cC$.
\item
If $b=0$, $\cA$ sends the register $R$ to $\cC$.
If $b=1$, $\cA$ applies a unitary $U_{ER}$ on the registers $E$ and $R$, and sends the register $R$ to $\cC$.
\end{enumerate}
Let $p_b$ be the probability that $\cC$ opens to $b$.
In other words,
\begin{eqnarray*}
p_0&\seteq&\langle\psi_0|_{RC}\Tr_E(|\Psi\rangle\langle\Psi|_{ERC})|\psi_0\rangle_{RC},\\
p_1&\seteq&\langle\psi_1|_{RC}\Tr_E(U_{ER}|\Psi\rangle\langle\Psi|_{ERC}U_{ER}^\dagger)|\psi_1\rangle_{RC}.
\end{eqnarray*}
We say that the commitment scheme is statistically sum-binding if
$p_0+p_1\le 1+\negl(\lambda)$.
\end{definition}


==> hiding.tex <==
\begin{proof}
Let us consider the following security game, 
$\sfhyb{0}{}(b)$, which is the same as the original
experiment.
\begin{enumerate}
\item
The challenger $\cC$ generates
\begin{eqnarray*}
|\psi_b\rangle_{RC}=\frac{1}{\sqrt{2^{2m}}}
\frac{1}{\sqrt{2^n}}
\sum_{x,z\in\{0,1\}^m}
\sum_{k\in\{0,1\}^n}
|x,z,k\rangle_R\otimes(X^xZ^z)^b|\phi_k\rangle_C,
\end{eqnarray*}
and sends
the register $C$ to the adversary $\cA$.
\item
$\cA$ outputs $b'\in\{0,1\}$, which is the output of this hybrid.
\end{enumerate}

Let us define $\sfhyb{1}{}(b)$ as follows:
\begin{enumerate}
\item
If $b=0$, $\cC$ 
chooses a Haar random $m$-qubit state $|\psi\rangle\leftarrow\mu$, and sends it to $\cA$.
If $b=1$, $\cC$ generates
\begin{eqnarray*}
|\psi_1\rangle_{RC}=\frac{1}{\sqrt{2^{2m}}}
\frac{1}{\sqrt{2^n}}
\sum_{x,z\in\{0,1\}^m}
\sum_{k\in\{0,1\}^n}
|x,z,k\rangle_R\otimes(X^xZ^z)|\phi_k\rangle_C,
\end{eqnarray*}
and sends
the register $C$ to $\cA$.
\item
$\cA$ outputs $b'\in\{0,1\}$, which is the output of this hybrid.
\end{enumerate}

\begin{lemma}
\begin{eqnarray*}
\left|\Pr[\sfhyb{0}{}(b)=1]-\Pr[\sfhyb{1}{}(b)=1]\right|\le \negl(\lambda)
\end{eqnarray*}
for each $b\in\{0,1\}$.
\end{lemma}

\begin{proof}
It is clear that $\Pr[\sfhyb{0}{}(1)=1]=\Pr[\sfhyb{1}{}(1)=1]$.
Let us show $|\Pr[\sfhyb{0}{}(0)=1]-\Pr[\sfhyb{1}{}(0)]|\le \negl(\lambda)$.
To show it, assume that 
$|\Pr[\sfhyb{0}{}(0)=1]-\Pr[\sfhyb{1}{}(0)=1]|$ is non-negligible.
Then, we can construct an adversary $\cA'$ that breaks the security of PRS.
The challenger $\cC'$ of the security game of PRS sends $\cA'$
$\frac{1}{2^n}\sum_k|\phi_k\rangle\langle\phi_k|$ if $b''=0$ 
and a Haar random state $|\psi\rangle\leftarrow \mu$ if $b''=1$.
$\cA'$ sends the state to the challenger $\cC$. $\cC$ sends the state to $\cA$.
$\cA'$ outputs the output of $\cA$. 
If $b''=0$, it simulates $\sfhyb{0}{}(0)$.
If $b''=1$, it simulates $\sfhyb{1}{}(0)$.
Therefore, $\cA'$ breaks the security of the PRS. 
\end{proof}

Let us define $\sfhyb{2}{}(b)$ as follows:
\begin{enumerate}
\item
The challenger $\cC$
chooses a Haar random $m$-qubit state $|\psi\rangle\leftarrow\mu$, and sends it to the adversary.
\item
The adversary outputs $b'\in\{0,1\}$, which is the output of this hybrid.
\end{enumerate}

\begin{lemma}
\begin{eqnarray*}
|\Pr[\sfhyb{1}{}(b)=1]-\Pr[\sfhyb{2}{}(b)=1]|\le \negl(\lambda)
\end{eqnarray*}
for each $b\in\{0,1\}$.
\end{lemma}

\begin{proof}
$\Pr[\sfhyb{1}{}(0)=1]=\Pr[\sfhyb{2}{}(0)=1]$ is clear.
Let us show $|\Pr[\sfhyb{1}{}(1)=1]-\Pr[\sfhyb{2}{}(1)=1]|\le \negl(\lambda)$.
To show it, assume that 
$|\Pr[\sfhyb{1}{}(1)=1]-\Pr[\sfhyb{2}{}(1)=1]|$ is non-negligible.
Then, we can construct an adversary $\cA'$ that breaks the security of PRS.
The challenger $\cC'$ of the security game of PRS sends $\cA'$
$\frac{1}{2^n}\sum_k|\phi_k\rangle\langle\phi_k|$ if $b''=0$ and 
a Haar random state $|\psi\rangle\leftarrow \mu$ if $b''=1$.
$\cA'$ applies $X^xZ^z$ with random $(x,z)\in\bit^n\times\bit^n$, 
and sends the state to $\cC$. $\cC$ sends the state to $\cA$.
$\cA'$ outputs the output of $\cA$. 
If $b''=0$, it simulates $\sfhyb{1}{}(1)$.
If $b''=1$, it simulates $\sfhyb{2}{}(1)$.
Therefore, $\cA'$ breaks the security of the PRS. 
\end{proof}

It is obvious that $\Pr[\sfhyb{2}{}(0)=1]=\Pr[\sfhyb{2}{}(1)=1]$.
Therefore we conclude
$|\Pr[\sfhyb{0}{}(0)=1]-\Pr[\sfhyb{0}{}(1)=1]|\le\negl(\lambda)$.
\end{proof}

==> oldconstruction.tex <==
\section{Construction2}
The commit phase is the following.
\begin{enumerate}
\item
The receiver chooses $x,z\leftarrow\{0,1\}^m$, and sends them to the sender.
\item
The sender generates 
\begin{eqnarray*}
|\psi_b\rangle:=\frac{1}{\sqrt{2^n}}\sum_{k\in\{0,1\}^n}|k\rangle_R\otimes(X^xZ^z)^b|\phi_k\rangle_C.
\end{eqnarray*}
The sender sends the register $C$ to the receiver.
\end{enumerate}
The open phase is the following.
\begin{enumerate}
\item
The sender sends the register $R$ and the bit $b$.
\item
The receiver checks the state is $|\psi_b\rangle$. If so, output $b$. If not, output $\bot$.
\end{enumerate}

\begin{lemma}[Hiding]
The construction satisfies hiding.
\end{lemma}
\begin{proof}
When the sender commits $b=0$, the state that receiver has is $\frac{1}{2^n}\sum_k|\phi_k\rangle\langle\phi_k|$,
which is computationally indistinguishable from Haar random states.
When the sender commits $b=1$, the state that receiver has is $\frac{1}{2^n}\sum_kX^xZ^z|\phi_k\rangle\langle\phi_k|X^xZ^z$.
\end{proof}

\begin{lemma}[Binding]
The construction satisfies binding.
\end{lemma}

\begin{proof}
Without loss of generality, we can assume that the malicious sender acts as follows:
\begin{enumerate}
\item
The receiver chooses $x,z\leftarrow\{0,1\}^m$, and sends them to the sender.
\item
The sender generates a state $\sigma_{RC}^{x,z}$, which depends on $(x,z)$, on the registers $R$ and $C$.
The sender sends the register $C$ to the receiver. 
\item
If the sender wants to make the receiver open $0$, the sender sends the register $R$ to the receiver. 
\item
If the sender wants to make the receiver open $1$, the sender applies a unitary $U_R^{x,z}$, which depends
on $(x,z)$, on the register $R$ and sends the register $R$ to the receiver.
\end{enumerate}
The probability $p_0$ that the receiver outputs $0$ is
\begin{eqnarray*}
p_0&:=&
\frac{1}{2^{2m}}\sum_{x,z}\Big(\frac{1}{\sqrt{2^n}}\sum_k\langle k|_R\langle \phi_k|_C\Big)
\sigma_{RC}^{x,z}
\Big(\frac{1}{\sqrt{2^n}}\sum_k|k\rangle_R|\phi_k\rangle_C\Big)\\
&=&\frac{1}{2^{2m}}\sum_{x,z}
F\Big(\frac{1}{\sqrt{2^n}}\sum_k|k\rangle_R|\phi_k\rangle_C,\sigma_{RC}^{x,z}\Big)\\
&\le& \frac{1}{2^{2m}}\sum_{x,z}F\Big(
\frac{1}{2^n}\sum_k|\phi_k\rangle\langle\phi_k|, \mbox{Tr}_R[\sigma_{R,C}^{x,z}]
\Big).
\end{eqnarray*}
The probability $p_1$ that the receiver outputs $1$ is
\begin{eqnarray*}
p_1
&:=&
\frac{1}{2^{2m}}\sum_{x,z}\Big(\frac{1}{\sqrt{2^n}}\sum_k\langle k|_R\langle \phi_k|_CX^xZ^z\Big)
(U_R^{x,z}\otimes I_C)\sigma_{RC}^{x,z}(U_R^{x,z\dagger}\otimes I_C)
\Big(\frac{1}{\sqrt{2^n}}\sum_k|k\rangle_RX^xZ^z|\phi_k\rangle_C\Big)\\
&=&
\frac{1}{2^{2m}}\sum_{x,z}F\Big(
\frac{1}{\sqrt{2^n}}\sum_k|k\rangle_RX^xZ^z|\phi_k\rangle_C,
(U_R^{x,z}\otimes I_C)\sigma_{RC}^{x,z}(U_R^{x,z\dagger}\otimes I_C)\Big)\\
&\le& \frac{1}{2^{2m}}\sum_{x,z}F\Big(
\frac{1}{2^n}\sum_kX^xZ^z|\phi_k\rangle\langle\phi_k|X^xZ^z, \mbox{Tr}_R[\sigma_{R,C}^{x,z}]
\Big).
\end{eqnarray*}
Then, we have
\begin{eqnarray*}
p_0+p_1
&\le&
1+\frac{1}{2^{2m}}\sum_{x,z}\sqrt{F\Big(
\frac{1}{2^n}\sum_k|\phi_k\rangle\langle\phi_k|, 
\frac{1}{2^n}\sum_kX^xZ^z|\phi_k\rangle\langle\phi_k|X^xZ^z
\Big)}\\
&\le&
1+\sqrt{F\Big(
\frac{1}{2^{2m}}\sum_{x,z}\frac{1}{2^n}\sum_k|\phi_k\rangle\langle\phi_k|, 
\frac{1}{2^{2m}}\sum_{x,z}\frac{1}{2^n}\sum_kX^xZ^z|\phi_k\rangle\langle\phi_k|X^xZ^z
\Big)}\\
&\le&
1+\sqrt{F\Big(
\frac{1}{2^n}\sum_k|\phi_k\rangle\langle\phi_k|, 
\frac{I^{\otimes m}}{2^m}
\Big)}\\
&\le&1+\frac{2^n}{\sqrt{2^m}}\\
&\le&1+\frac{1}{2^{\frac{n}{2}}}.
\end{eqnarray*}

\end{proof}


==> preamble_packages.tex <==
\usepackage{graphicx}% Include figure files
\usepackage{bm}
\usepackage{amsmath,amssymb,fancybox}
\usepackage{amscd,amsfonts}
\usepackage{theorem}
\usepackage{color}




\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}




\usepackage[dvipsnames]{xcolor}
\definecolor{darkblue}{rgb}{0,0,0.6}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{maroon}{rgb}{0.5,0.1,0.1}
\definecolor{dpurple}{rgb}{0.2,0,0.65}
\definecolor{darkviolet}{RGB}{130,95,141}

\usepackage
[pdfpagelabels=true,
linktocpage=false,
bookmarks=true,bookmarksnumbered=false,bookmarkstype=toc,
pagebackref,
colorlinks=true,linkcolor=darkblue,urlcolor=darkblue,citecolor=darkviolet]
{hyperref}


\usepackage[capitalise,noabbrev]{cleveref}
\usepackage{mathtools}
\usepackage[absolute]{textpos}
\usepackage[final]{microtype}
\usepackage[absolute]{textpos}
\usepackage{everypage}
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{etex}
\usepackage{graphicx,pstricks}
\usepackage{centernot}
\usepackage{xspace}
\usepackage{pifont}
\usepackage{paralist}
\usepackage{booktabs}
\usepackage{dashbox}
\usepackage{lscape}
\usepackage{colortbl}


==> references.tex <==
\begin{thebibliography}{00}
\bibitem{Blu81}
M. Blum, 
Coin flipping by telephone. 
In Allen Gersho, editor, Advances in Cryptology:
A Report on CRYPTO 81, CRYPTO 81, IEEE Workshop on Communications Security, Santa
Barbara, California, USA, August 24-26, 1981, pages 11–15. U. C. Santa Barbara, Dept. of Elec.
and Computer Eng., ECE Report No 82-04, 1981.


\bibitem{Nao91} 
M. Naor, 
Bit commitment using pseudorandomness.
Journal of cryptology, pages 151–158, 1991.

\bibitem{HILL99}
J. H{\aa}stad, R. Impagliazzo, L. A. Levin, and M. Luby,
A Pseudorandom Generator from any One-way Function.
SIAM J. Comput. {\bf28}(4) pages 1364-1396, 1999.

\bibitem{Goldreich_textbook}
O. Goldreich, 
Foundations of Cryptography.
Cambridge University Press. 2004.

\bibitem{LR86} 
M. Luby and C. Rackoff, 
Pseudo-random permutation generators and cryptographic
composition. In 18th ACM STOC, pages 356–363. ACM Press, May 1986.

\bibitem{IL89} 
R. Impagliazzo and M. Luby, 
One-way functions are essential for complexity based
cryptography (extended abstract). In 30th FOCS, pages 230–235. IEEE Computer Society Press,
October / November 1989.

\bibitem{ILL89} 
R. Impagliazzo, L. A. Levin, and M. Luby, 
Pseudo-random generation from
one-way functions (extended abstracts). In 21st ACM STOC, pages 12–24. ACM Press, May
1989.

\bibitem{BB84}
C. H. Bennett and G. Brassard, 
Quantum cryptography: Public key distribution and coin tossing. In IEEE International Conference on Computers 
Systems and Signal Processing, pages 175–179. IEEE, 1984.

%\bibitem{OT} 
%Oblivious transfer is the following task:
%Alice has two messages $m_0,m_1$. 
%Bob can learn one of them, but he cannot learn the other. Alice cannot learn which message Bob learns. 

\bibitem{BCKM21}
J. Bartusek, A. Coladangelo, D. Khurana, and F. Ma, 
One-way functions imply secure computation in a quantum world. 
In Tal Malkin and Chris Peikert, editors, CRYPTO 2021, Part I, volume 12825 of LNCS, pages 467–496, Virtual Event, August 2021. Springer, Heidelberg.

\bibitem{BLSV19}
A. B. Grilo, H. Lin, F. Song, and V. Vaikuntanathan,
Oblivious Transfer Is in MiniQCrypt. In: Canteaut and Standaert (eds) 
Advances in Cryptology - EUROCRYPT 2021. 
EUROCRYPT 2021. Lecture Notes in Computer Science, vol 12697. Springer, Cham. 


\bibitem{CK88} 
C. Cr\'{e}peau and J. Kilian, 
Achieving oblivious transfer using weakened security assumptions (extended abstract). 
In 29th FOCS, pages 42-52. IEEE Computer Society Press, October 1988.

\bibitem{BBCS92} 
C. H. Bennett, G. Brassard, C. Cr\'{e}peau, and M.-H. Skubiszewska, 
Practical quantum oblivious transfer. In Joan Feigenbaum, editor, CRYPTO’91, volume 576 of LNCS,
pages 351-366. Springer, Heidelberg, August 1992.

\bibitem{MS94} 
D. Mayers and L. Salvail, 
Quantum oblivious transfer is secure against all individual
measurements. In Proceedings Workshop on Physics and Computation. PhysComp’94, pages 69-77.
IEEE, 1994.

\bibitem{Yao95} 
A. C.-C. Yao, 
Security of quantum protocols against coherent measurements. In 27th
ACM STOC, pages 67-75. ACM Press, May / June 1995.

\bibitem{DFL+09} 
I. Damgard, S. Fehr, C. Lunemann, L. Salvail, and C. Schaffner, 
Improving the security of quantum protocols via commit-and-open. In Shai Halevi, editor,
CRYPTO 2009, volume 5677 of LNCS, pages 408-427. Springer, Heidelberg, August 2009.

\bibitem{IR90}
R. Impagliazzo and S. Rudich, 
Limits on the provable consequences of one-way permutations. 
In Shafi Goldwasser, editor, CRYPTO’88, volume 403 of LNCS, pages 8-26. Springer, Heidelberg, August 1990.

\bibitem{black-box}

\bibitem{LC97} 
H.-K. Lo and H. F. Chau, 
Is quantum bit commitment really possible?
Phys. Rev. Lett. {\bf78}, 3410–3413 (1997).

\bibitem{May97} 
D. Mayers, 
Unconditionally secure quantum bit commitment is impossible.
Phys. Rev. Lett. {\bf78}, 3414–3417 (1997).
\bibitem{YWLQ15} 
J. Yan, J. Weng, D. Lin, and Y. Quan,  
Quantum bit commitment with application in quantum zero-knowledge proof (extended abstract). In Khaled M. Elbassioni and Kazuhisa Makino, editors, Algorithms and Computation - 26th International Symposium, ISAAC 2015, Nagoya, Japan, December 9-11, 2015, Proceedings, volume 9472 of Lecture Notes in Computer Science, pages 555–565. Springer, 2015.


\bibitem{DMS00}
P. Dumais, D. Mayers, and L. Salvail. 
Perfectly concealing quantum bit commitment from any quantum one-way permutation. 
In EUROCRYPT, pages 300-315, 2000.

\bibitem{CLS01}
C. Cr{\'{e}}peau, F. L{\'{e}}gar{\'{e}} and L. Salvail,
How to convert the flavor of a quantum bit commitment.
In EUROCRYPT, pages 60-77, 2001.

\bibitem{KO09}
T. Koshiba and T. Odaira, 
Statistically-hiding quantum bit commitment from approximable-preimage-size quantum one-way function. 
In Andrew M. Childs and Michele Mosca, editors, Theory of Quantum Computation, Communication, and Cryptography, 4th Workshop, TQC 2009, Waterloo, Canada, May 11-13, 2009, Revised Selected Papers, volume 5906 of Lecture Notes in Computer Science, pages 33–46. Springer, 2009.

\bibitem{KO11}
T. Koshiba and T. Odaira, 
Non-interactive statistically-hiding quantum bit commitment from any quantum one-way function.
arXiv:1102.3441, 2011.

\bibitem{Yan20}
J. Yan, 
General Properties of Quantum Bit Commitments.
Cryptology ePrint Archive: Report 2020/1488

\bibitem{BB21}
N. Bitansky and Z. Brakerski,
Classical Binding for Quantum Commitments.
TCC 2021

\bibitem{DiffieHellman}
W. Diffie and M. Hellman, 
New directions in cryptography, 
in IEEE Transactions on Information Theory, vol.22, no.6, pp.644-654, 
November 1976. 

\bibitem{Gottesman_Chuang}
D. Gottesman and I. L. Chuang,
Quantum Digital Signatures.
arXiv:quant-ph/0105032.


\bibitem{JLS18} 
Z. Ji, Y.-K. Liu, and F. Song, 
Pseudo-random quantum states. 
In Hovav Shacham and Alexandra Boldyreva, editors, CRYPTO 2018, Part III, volume 10993 of LNCS, pages 126–152. Springer, Heidelberg, August 2018.
\bibitem{BS1}
Z. Brakerski and O. Shmueli, 
(Pseudo) Random Quantum States with Binary Phase. 
In: Hofheinz and Rosen (eds) Theory of Cryptography. TCC 2019. 
Lecture Notes in Computer Science, vol 11891. Springer, Cham. 

\bibitem{BS2}
Z. Brakerski and O. Shmueli, 
Scalable Pseudorandom Quantum States. 
In: Micciancio and Ristenpart (eds) Advances in Cryptology - CRYPTO 2020. 
Lecture Notes in Computer Science, vol 12171. Springer, Cham. 

\bibitem{Kre21} 
W. Kretschmer,
Quantum pseudorandomness and classical complexity.
16th Conference on the Theory of Quantum Computation, Communication and Cryptography (TQC 2021), 
Leibniz International Proceedings inInformatics (LIPIcs), 197:2:1–2:20, 2021



\bibitem{MP12} 
M. Mahmoody and R. Pass,
The curious case of non-interactive commitments - on the power of black-box vs. non-black-box use of primitives.
In Reihaneh SafaviNaini and Ran Canetti, editors, CRYPTO 2012, volume 7417 of LNCS, pages 701–718. Springer, Heidelberg, August 2012.


\bibitem{Unr16}
D. Unruh,
Collapse-binding quantum commitments without random oracles.
Asiacrypt 2016.

\bibitem{FUYZ20}
J. Fang, D. Unruh, J. Yan, and D. Zhou,
How to Base Security on the Perfect/Statistical Binding Property of Quantum Bit Commitment?
Cryptology ePrint Archive, Report 2020/621, 2020

\bibitem{BCKM_QCOM}
Indeed, Ref.~\cite{BCKM21} states as follows: 
``\emph{Moreover if in the future, new constructions of statistically binding, quantum computationally hiding commitments involving quantum communication are discovered based on assumptions weaker
than quantum-hard one-way functions, it would be possible to plug those into our protocol compilers to
obtain QOT.}"
Unfortunately, our commitment scheme cannot be directly plugged into their construction since they require \emph{classical binding} property~\cite{BB21}, which is stronger than the standard notion of binding for quantum commitments proven in this paper. 


\bibitem{Kre21explain}
Ref.~\cite{Kre21} gives only the case when $m=n$, but it is clear that
the result holds for $m\ge cn$ with constant $c>1$. 


\bibitem{Lamport}
L. Lamport,
Constructing Digital Signatures from a One Way Function. 
SRI International (CSL-98). Retrieved 17 February 2021.

\bibitem{Kawachi}
A. Kawachi, T. Koshiba, H. Nishimura, and T. Yamakami,
Computational Indistinguishability Between Quantum
States and Its Cryptographic Application.
J. Cryptol. 25: 528–555 (2012).

\bibitem{LWEPKE}
J. Doliskani,
Efficient Quantum Public-Key Encryption
From Learning With Errors.
arXiv:2105.12790.

\bibitem{AQY}
P. Ananth, L. Qian, and H. Yuen,
Cryptography from pseudorandom quantum states.
Cryptology ePrint Archive: Report 2021/1663

\bibitem{AQY_personal_communication}
P. Ananth, L. Qian, and H. Yuen,
personal communication

\bibitem{simple_example}
In fact, the security proofs of the constructions of Refs.~\cite{JLS18,BS1}
are simpler for $t=1$. Furthermore, there is a simple construction of PRS for $t=1$ by
using a pseudorandom generator $G:\{0,1\}^n\to\{0,1\}^m$. 
In fact, we have only to take $|\phi_k\rangle=|G(k)\rangle$.


\bibitem{another_construction}
Another example of constructions is 
$|\psi_0\rangle=\sum_{k\in\{0,1\}^n}|k\rangle|\phi_k\rangle$
and
$|\psi_1\rangle=\sum_{r\in\{0,1\}^m}|r\rangle|r\rangle$.
We have chosen the one we have explained, because
the analogy to Naor's commitment scheme is clearer.

\bibitem{Wilde}
M. Wilde,
From Classical to Quantum Shannon Theory.
arXiv:1106.1445

\bibitem{NayakShor}
A. Nayak and P. Shor,
Bit-commitment-based quantum coin flipping.
Phys. Rev. A {\bf 67}, 012304 (2003).


\end{thebibliography}
